Hole in one: Pathways to deterministic single-acceptor incorporation in Si(100)-2$\times$1

Stochastic incorporation kinetics can be a limiting factor in the scalability of semiconductor fabrication technologies using atomic-precision techniques. While these technologies have recently been extended from donors to acceptors, the extent to which kinetics will impact single-acceptor incorporation has yet to be assessed. We develop and apply an atomistic model for the single-acceptor incorporation rates of several recently demonstrated precursor molecules: diborane (B$_2$H$_6$), boron trichloride (BCl$_3$), and aluminum trichloride in both monomer (AlCl$_3$) and dimer forms (Al$_2$Cl$_6$), to identify the acceptor precursor and dosing conditions most likely to yield deterministic incorporation. While all three precursors can achieve single-acceptor incorporation, we predict that diborane is unlikely to achieve deterministic incorporation, boron trichloride can achieve deterministic incorporation with modest heating (50 $^{\circ}$C), and aluminum trichloride can achieve deterministic incorporation at room temperature. We conclude that both boron and aluminum trichloride are promising precursors for atomic-precision single-acceptor applications, with the potential to enable the reliable production of large arrays of single-atom quantum devices.

==> sm.tex <==
% Supplementary information starts here
\clearpage
\widetext
\begin{center}
\textbf{\large Supplementary information: Pathways to deterministic atomic-precision single acceptor incorporation on Si(100)2$\times$1}
\end{center}

% Reset counters and add an S prefix on equation and figure numbers
\setcounter{section}{0}
\setcounter{page}{1}
\makeatletter

% This is Andrew's ongoing rewrite of the SM.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Contents}

The Supplemental Materials elaborate on details of some of the central results in the main body of the paper.
\begin{itemize}
    \item Appendix A describes...
\end{itemize}

\section*{Appendix A: }
\setcounter{equation}{0}
\setcounter{figure}{0}
\renewcommand{\theequation}{A\arabic{equation}}
\renewcommand{\thefigure}{A\arabic{figure}}
\label{app:expt_details}

